AntLM: Bridging Causal and Masked Language Models

Causal Language Modeling (CLM) and Masked Language Modeling (MLM) are two mainstream learning paradigms based on Transformer networks, specifically the Decoder-only and Encoder-only architectures. The strengths of each paradigm in downstream tasks have shown a mix of advantages and disadvantages. In the past BabyLM Challenge 2023, although the MLM paradigm achieved the best average performance, the CLM paradigm demonstrated significantly faster convergence rates. For the BabyLM Challenge 2024, we propose a novel language modeling paradigm named $\textbf{AntLM}$, which integrates both CLM and MLM to leverage the advantages of these two classic paradigms. We chose the strict-small track and conducted experiments on two foundation models: BabyLlama, representing CLM, and LTG-BERT, representing MLM. During the training process for specific foundation models, we alternate between applying CLM or MLM training objectives and causal or bidirectional attention masks. Experimental results show that combining the two pretraining objectives leverages their strengths, enhancing overall training performance. Under the same epochs, $AntLM_{BabyLlama}$ improves Macro-average by 1%, and $AntLM_{LTG-BERT}$ achieves a 2.2% increase over the baselines.

==> arxiv/fig/fig_example.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth} % 每张图片占用的宽度
        \includegraphics[width=\linewidth]{fig/blimp_filter.pdf}
      \caption{BLiMP}
        \label{fig:sub1}
    \end{subfigure}
    % \begin{subfigure}{0.3\textwidth}
    %     \includegraphics[width=\linewidth]{fig/blimp_supplement.pdf}
    %     \caption{BLiMP Supplement}
    %     \label{fig:sub2}
    % \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{fig/ewok.pdf}
        \caption{EWok}
        \label{fig:sub3}
    \end{subfigure}
    % 在三个数据集上分阶段的实验结果。在BabyLlama基座上“3\_CLM+ 8\_MLM+2\_CLM+8\_MLM+ 2\_CLM ”的每个阶段的评估折线图
    % 训练阶段之间测评结果不连续的原因是我们使模型在不同的训练任务阶段均使用对应训练任务类别的测评方法。
    \caption{The phased experimental results on three datasets. The evaluation line chart for each stage of ``3\_\colorbox{CLM}{CLM} + 8\_\colorbox{MLM}{MLM} + 2\_\colorbox{CLM}{CLM} + 8\_\colorbox{MLM}{MLM} + 3\_\colorbox{CLM}{CLM}'' on the BabyLlama model. The reason for the discontinuity in evaluation results between training phases is that we applied the evaluation method corresponding to the specific task categories at each stage of the training process.}
    \label{fig:example}
\end{figure*}


==> arxiv/fig/fig_main.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/fig_arch.pdf}
  \caption{A diagram of AntLM$_\text{LTG-BERT}$. Based on the LTG-BERT architecture, we propose a joint MLM and CLM training objective. It is worth noting that the two objectives fully share parameters, but differ in their attention masks. The diagram also applies to AntLM$_\text{BabyLlama}$, with the difference in the architecture (e.g., positional encoding and the activation function of GLU).}
  \label{fig:main}
\end{figure}


==> arxiv/sec/1_abstract.tex <==
% 最后写
% 在BabyLM的挑战赛中，我们提出集成Masked Language Modeling（MLM）和Causal Language Modeling (CLM)两种预训练目标的模型——AntLM。我们尝试了分别选取BabyLlama和LTG-BERT作为基座模型在strict-small track上进行了实验。通过修改预训练目标，BabyLlama比baselines在Macroaverage高了平均1个point，LTG-BERT比baselines高了平均7个points。实验结果显示通过集成两种预训练目标，可以对模型的训练起到积极的影响。%
Causal Language Modeling (CLM) and Masked Language Modeling (MLM) are two mainstream learning paradigms based on Transformer networks, specifically the Decoder-only and Encoder-only architectures. 
The strengths of each paradigm in downstream tasks have shown a mix of advantages and disadvantages. 
In the past BabyLM Challenge 2023, although the MLM paradigm achieved the best average performance, the CLM paradigm demonstrated significantly faster convergence rates.
For the BabyLM Challenge 2024, we propose a novel language modeling paradigm named \textbf{AntLM}, which integrates both CLM and MLM to leverage the advantages of these two classic paradigms.
% In the BabyLM Challenge 2024, we propose AntLM, which integrates two classic language modeling paradigms: Causal Language Modeling (CLM) and Masked Language Modeling (MLM). 
We chose the strict-small track and conducted experiments on two foundation models: BabyLlama, representing CLM, and LTG-BERT, representing MLM.
% We conducted experiments in the strict-small track using BabyLlama and LTG-BERT as the base models.
During the training process for specific foundation models, we alternate between applying CLM or MLM training objectives and causal or bidirectional attention masks.
% BabyLlama, as an autoregressive model, predicts the next token using causal masking, while LTG-BERT, a bidirectional encoder, leverages MLM by masking 15\% of tokens and using context to predict the original tokens. 
% We dynamically adjust attention mechanisms to enable switching between these tasks during pre-training. 
% The experimental results indicate that these two pretraining objectives demonstrate distinct advantages across different datasets. Integrating them allows for the strengths of each objective to be fully leveraged, resulting in a positive impact on the final model’s training performance. Further experiments reveal that, under the same number of epochs, BabyLlama outperforms the baselines by an average of 1 point in Macro-average, while LTG-BERT achieves an average improvement of 2 points over the baselines.
Experimental results show that combining the two pretraining objectives leverages their strengths, enhancing overall training performance. 
Under the same epochs, AntLM$_\text{BabyLlama}$ improves Macro-average by 1\%, and AntLM$_\text{LTG-BERT}$ achieves a 2.2\% increase over the baselines.

==> arxiv/sec/2_intro.tex <==
\section{Introduction}
\label{sec:intro}
% P1: 介绍LM的背景、发展、应用
%近年来，随着研究不断开展，LM迎来了迅速发展，逐渐演变为复杂和强大的神经网络模型，即大语言模型（LLM）。语言模型（LM）是自然语言处理（NLP）领域的核心技术之一，它通过对语言序列进行概率建模，然后可以用于生成任务（如机器翻译、人机问答）或下游分类任务（如情感分类）中。越来越大的语言模型在各个基准上不断取得了新的突破。然而，模型规模的增加，使得语言模型训练所需的计算能力和训练数据量变得巨大，缺少计算资源的个人或团体难以负担这样的训练过程。因此，如何用更少的数据计算量进行高效轻量的LM训练是值得被研究的。%
% Recently, with the ongoing advancement of research, Language Models (LM) have seen rapid development, gradually evolving into complex and powerful neural network models known as Large Language Models (LLMs). LMs are one of the core technologies in the field of Natural Language Processing (NLP), as they model language sequences probabilistically, enabling their use in generative tasks (machine translation and question answering) as well as downstream classification tasks (sentiment analysis). Larger and larger language models have continuously set new benchmarks across various tasks. However, as the size of these models grows, the computational power and the amount of training data required have also surged 
% ~\cite{bender2021dangers}, making it difficult for individuals or groups with limited computational resources to bear the cost of such training processes. Therefore, researching efficient and lightweight LM training with reduced data and computational demands is crucial.

% Language Models (LMs) play a significant role in Natural Language Processing (NLP). 
% They are integral in a variety of applications, such as machine translation~\cite{hendy2023good}, speech recognition~\cite{prabhavalkar2023end}, sentiment analysis~\cite{tan2023survey}, and information extraction~\cite{wei2023zero}, wherein they leverage the ability to understand, generate, and summarize text data.

Language Modeling (LM) is a core task in NLP and a key technology for natural language understanding and generation, supporting a wide range of applications including machine translation~\cite{hendy2023good}, speech recognition~\cite{prabhavalkar2023end}, sentiment analysis~\cite{tan2023survey}, and information extraction~\cite{wei2023zero}.
% In the past years, LM has seen significant development, evolving from simple models such as n-gram models to more complex models like Recurrent Neural Networks (RNNs), Long Short Term Memory (LSTMs), and more recently, Transformer-based models like GPT~\cite{gpt2} and BERT~\cite{devlin2018bert}. These models have shown unprecedented performance in generating and comprehending natural language.
Over the past decades, LM has seen significant development, evolving from simple models like n-grams~\cite{ngram} to more sophisticated models, such as recurrent neural networks~\cite{rnn}, long short-term memory networks~\cite{lstm}, and more recently, Transformer-based large language models (LLMs) like GPT~\cite{gpt2} and BERT~\cite{devlin2018bert}. 
LLMs have demonstrated human-like or even superhuman performance in language modeling.

However, the tremendous success of LLMs relies on learning from massive corpora, which is not as data-efficient and low-energy as human language learning.
The BabyLM Challenge 2023~\cite{warstadt2023papersbabylmchallenge} and 2024~\cite{choshen2024callpapers2ndbabylm} is a shared task over two consecutive years. 
It aims to encourage the discovery of more effective methods for training models using limited data.
Considering that a 13-year-old child has encountered fewer than 100 million words in their lifetime, the shared task has introduced the \textit{strict-small track}\footnote{Due to limitations in computational resources, we have not yet explored the \textit{strict track} and the \textit{multimodal track}.}.
These tracks confine pre-training data to 10 million and 100 million words. 
These datasets consist of child-accessible materials, such as books, conversations, and Wikipedia entries, to enhance the relevance of language model pre-training to human language learning processes. Compared to 2023, the 2024 competition removed the Children’s Book Test~\cite{Childrens_Book_Test} and QCRI Educational Domain Corpus datasets~\cite{QED}. The 2024 competition also reduced the proportion of OpenSubtitles~\cite{OpenSubtitles} dataset while increasing the proportions of CHILDES~\cite{CHILDES} and Project Gutenberg~\cite{Gutenberg} datasets.




% As the models grow larger and more complex, they pave the way for performance improvements across various NLP tasks. However, the increase in model size incurs a proportional surge in computational resources and training data required~\cite{bender2021dangers}. Hence, developing methods to train LMs more efficiently with a lower computational budget is critical and these methods would democratize the use of advanced AI technologies by allowing individuals and smaller entities to take part in model training and development.

% P2: 介绍BabyLM目标、任务、意义
%BabyLM Challenge 2024是一项共享任务，旨在鼓励大家发掘更有效的从有限数据中使得模型学习的方法。考虑到一个13岁的孩子在他所活过的时间里看到的单词少于1亿个，现存效果突出的模型预训练使用的单词数量要比这个数字高出几个数量级，并且通常都是通过精挑细选的优质数据。在这种情况下，BabyLM 设置了 strict-small track 和 strict track 赛道，分别限制了 10 million 和 100 million 的预训练数据，并且这些数据覆盖儿童能够轻易接受的读物、对话和维基百科等等，以此希望提高语言模型预训练和人类语言学习过程的相关性，并鼓励参与者探索适用于语言模型更有效的和数据效率更高的训练算法，使得可以在更小的训练预算上解决研究问题。%
% BabyLM Challenge 2024~\cite{choshen2024callpapers2ndbabylm} is a shared task to encourage the discovery of more effective methods for training models using limited data. Considering that a 13-year-old child has encountered fewer than 100 million words in their lifetime, the number of words used for pre-training in most high-performing models exceeds this by several orders of magnitude, typically drawn from carefully curated high-quality data. In this context, BabyLM Challenge 2024 has introduced the \textit{strict-small track} and the \textit{strict track}. These tracks confine pre-training data to 10 million and 100 million words, respectively. These datasets consist of child-accessible materials, such as books, conversations, and Wikipedia entries, to enhance the relevance of language model pre-training to human language learning processes. The challenge encourages participants to explore more effective and data-efficient training algorithms for language models, enabling them to tackle research problems with smaller training budgets.

% P3: 介绍LM两种主流建模方式及其各自特点，提出问题：是否能融合两者进行语言建模？
%在当前的语言模型的研究中，主流的两个建模方式是掩码语言模型和自回归语言模型。掩码语言模型的代表是BERT等模型。通过在输入文本中随机选择部分token替换为[MASK]，然后训练模型去预测原来的token。这种建模方式通过全局信息建模，在需要捕捉双向语境信息的任务（如文本分类）上表现优异。自回归语言模型的代表是GPT等模型，通过给定上文，预测下一个token的方式来训练。自回归语言模型在生成任务上的表现强大。鉴于两种建模方法的优势，本文提出一个问题：能否融合两种建模方式？%
The current investigation of LMs primarily adopts two predominant modeling paradigms: Causal Language Models (CLMs), represented by GPT~\cite{gpt2}, and Masked Language Models (MLMs), represented by BERT~\cite{devlin2018bert}. CLMs employ next-token prediction as their training objective, which is predicting the next token given the preceding context, and they perform exceptionally well on generative tasks. On the other hand, the training objective of MLM is the random selection and masking of some tokens in the input text, following which the model is trained to predict the original unmasked tokens. Due to its global information modeling capabilities, this approach excels in tasks necessitating the capture of bidirectional contextual information, such as text classification. Considering these modeling paradigms' strengths, this paper raises an important question: Could the two modeling methodologies be seamlessly integrated?

% P4: 介绍我们的方法和结论
% 结论还没写
%直觉上讲，进行MLM任务使得模型在文本的深度双向编码上下文表示的方向进行学习，而CLM任务使得模型看过过去的内容再对文本预测生成方向进行学习，这两者的学习目标并不冲突，存在结合的可能。就像孩子学习一门新的语言时需要同时进行完形填空题型和写作题型的训练一样，模型的训练过程也可以采取多任务的形式，所以我们考虑使我们的模型同时在这两种任务上进行学习。为此，我们使用统一的模型架构，让模型在MLM和CLM两种任务上交替学习，尝试使得模型能模仿人类的学习过程，从而在少量文本数据中学习到更加深层次的知识体系。%
Intuitively, performing the MLM task allows the model to learn bidirectional contextual encoding of text, while the CLM task enables the model to predict and generate text based on prior content. These two learning objectives are not in conflict and could potentially be integrated. Analogous to a child learning a new language via practicing both cloze exercises and writing assignments, the training mechanism for a model can similarly employ a multi-task strategy. Therefore, we consider enabling our model to learn both tasks concurrently. To achieve this, we adopt a unified model architecture and alternate the training objective between MLM and CLM tasks. This approach attempts to mimic the human learning process, hence helping the model acquire deeper knowledge from a limited amount of text data.

% P5: 介绍本文贡献
% 为了观察集成MLM和CLM两个预训练任务对于模型性能的影响，我们分别使用LTG-BERT和LlaMa两种模型作为基座，在2024年的babylm的10M数据集上进行了测试。实验结果显示LTG-BERT和BabyLlama均在Macroaverage上得到了提升。通过实验，我们验证了集成两种目标可以对模型的训练起到积极的作用。 %
To examine the effect of integrating MLM and CLM pretraining tasks on model performance, we conducted experiments using LTG-BERT and BabyLlama\footnote{We only utilized the BabyLlama architecture and did not apply the knowledge distillation method here.} as base models, testing on the BabyLM2024 10M datasets. LTG-BERT, an Encoder-only model, and BabyLlama, a Decoder-only model, are notable architectures from the 2023 BabyLM Challenge .The results indicate that both LTG-BERT and BabyLlama showed improvements in macroaverage scores. These experiments confirm that the integration of these two pretraining objectives can positively impact model training.

==> arxiv/sec/3_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

% 自回归LM
%自回归语言模型（Causal Language Models, CLMs）在自然语言处理（NLP）的发展中起到了关键作用，尤其在涉及序列生成的任务中。OpenAI 提出的生成式预训练变换模型（Generative Pre-trained Transformer, GPT）是自回归语言模型应用的一个重要突破。GPT 通过基于所有前面的 tokens 来建模序列中每个 token 的概率，使其在文本补全、机器翻译和摘要生成等任务中表现优异。随后的 GPT-2 和 GPT-3 的发布进一步展示了扩展自回归语言模型的强大能力。这些模型通过增加参数数量和训练数据，在零样本和少样本学习等任务中设立了新的性能基准。GPT 系列模型牢固地确立了自回归模型在生成任务中的主导地位。最近，Meta 推出了 LLaMA（Large Language Model Meta AI）系列，证明了在比早期模型（如 GPT-3）更少的参数和计算资源下，也能够有效训练出功能强大的自回归语言模型（ALM）。LLaMA 专为学术研究的易获取性设计，保留了自回归框架，同时在一系列 NLP 任务中展现出具有竞争力的性能。 
\textbf{Causal Language Models} have played a pivotal role in the development of NLP, particularly in tasks involving sequence generation. The foundational work by OpenAI on the Generative Pre-trained Transformer (GPT)~\cite{gpt} marked a significant breakthrough in the use of CLMs for a variety of NLP applications. GPT~\cite{gpt} models the probability of each token in a sequence based on all preceding tokens, enabling it to perform well on tasks like text completion, machine translation, and summarization. The subsequent release of GPT-2~~\cite{gpt2} and GPT-3~\cite{gpt3} further illustrated the power of scaling CLMs. These models, with their increased parameter sizes and training data, have set new performance benchmarks in tasks like zero-shot and few-shot learning.  The GPT family firmly established the dominance of autoregressive models in generative tasks. More recently, Meta introduced the LLaMA~\cite{touvron2023llama} series, which demonstrated that highly capable CLMs could be trained efficiently on fewer parameters and less compute than earlier models like GPT-3. 
LLaMA, designed to be accessible for academic research, retains the autoregressive framework while achieving competitive performance across a range of NLP tasks. 


% MLM
%掩码语言模型（MLM）是为了实现训练模型的深度双向表示而使用的一种训练方式，也常被称为完形填空任务。具体来说，我们会用一个特殊token [MASK] 来随机屏蔽一定比例的输入token，然后使得模型预测这些被屏蔽的token。这项训练任务在Bert中被开创性的使用，并在后续的RoBERTa、ALBERT中得以沿用。MLM任务也在后续的工作中得以研究改进，例如SpanBERT使得模型在MLM任务中可以预测连续的词语而非单个token。%
\textbf{Masked Language Model} is a training approach used to develop deep bidirectional representations of context, often referred to as a cloze task~\cite{taylor1953cloze}. Specifically, a special token [MASK] is employed to randomly mask a proportion of input tokens, and the model is trained to predict these masked tokens. This training task was first innovatively introduced in BERT~\cite{devlin2018bert} and has been adopted in subsequent models like RoBERTa~\cite{liu2019roberta} and ALBERT~\cite{lan2019albert}. Research has also led to improvements in MLM tasks, such as in SpanBERT~\cite{joshi2020spanbert}, where the model is trained to predict spans of words instead of individual tokens, enhancing its ability to capture long-range dependencies.

% 上述的两种语言建模方式各有优劣，且有互补的可能，本文聚焦在探索新的关联两者的方法，并提供insights。
% The two language modeling approaches each have their strengths and weaknesses, with the potential for complementarity. This paper focuses on exploring novel methods to bridge the two and provides valuable insights.
% 统一建模 %
%统一建模是指使用统一的模型架构对多个训练任务和测评任务进行建模。在T5模型中，多种下游任务都被统一建模为了文本到文本的任务，极大增强了模型的多任务学习能力。不仅如此，许多相关工作也进行了对模型多任务训练和多任务测评的统一建模，使得其成为一种提高模型泛化能力的常用方法。%

\textbf{Unified modeling} refers to using a single model architecture to handle multiple training and evaluation tasks. In the T5~\cite{raffel2020exploringT5} model, various downstream tasks were reformulated as text-to-text tasks, significantly enhancing the model’s ability for multitask learning. Moreover, many related works~\cite{sanh2019hierarchicalUni1,liu2020attentionUni2} have also applied unified modeling for multitask training and evaluation, making it a common approach to improve the generalization ability of models.
% 基于Bert架构的UniLM是统一建模的重要尝试之一。UniLM通过使用特定的自注意力掩码来控制预测时使用的上下文信息。在预测token的时候，它不仅可以像自编码语言模型一样利用掩码标志的上下文进行训练，还可以像自回归语言模型一样从左向右的进行训练。此外，UniLM还可以像Encoder-Decoder架构的模型先对输入文本进行编码，再从左向右的生成序列。通过切换注意力矩阵即可完成训练任务的切换和下游应用场景的切换。%
UniLM~\cite{dong2019unified}, based on the BERT architecture, is one of the significant endeavors in unified modeling. By employing specific self-attention masks, UniLM controls the contextual information used during prediction. When predicting tokens, it not only trains like an autoencoding language model by leveraging the context of masked tokens but also performs left-to-right training like an autoregressive language model. Additionally, UniLM can function similarly to encoder-decoder architectures by encoding the first input text and then generating sequences from left to right. By switching the attention matrix, it seamlessly transitions between different training tasks and downstream application scenarios. 

% 现有方法已经从模型结构、参数共享方面统一了CLM和MLM网络，但是训练目标统一的研究仍然空白，本文是首个聚焦在训练目标统一的工作。
Existing methods have unified CLM and MLM networks regarding model architecture and parameter sharing.
However, research on unifying their training objectives remains unexplored. 
This paper is the first to bridge the two classic training objectives.

==> arxiv/sec/4_method.tex <==


\section{Methods}
\label{sec:method}

\subsection{Preliminaries}
\label{ssec:prel}
% BabyLlama结构+自回归训练目标 @yu
%本研究中我们其中一个模型以进行自回归语言模型的训练的 BabyLlama 为基座。BabyLlama 模型采用了经典的自回归预测任务，即在给定序列的前 n 个 token 后，预测第 n+1 个 token，自回归训练目标是最小化每个时间步预测下一个 token 的负对数似然。为实现这一目标，模型在自注意力机制中引入了因果掩码 (causal mask)，该掩码为一个下三角矩阵，确保每个 token 只能关注其前面的 token，形式上，给定一个长度为 $T$的输入序列, $x_1, x_2, \dots, x_T$，对应的注意力掩码 $M$ 为一个 T×T的下三角矩阵，即Mij表示注意力机制应该注意到的部分，当且仅当 i>=j，否则 Mij表示应该被掩码不应该注意的部分。这种掩码方式有效防止了模型在训练时泄露未来的信息，从而有效捕获序列的顺序性和依赖关系。

BabyLlama~\cite{timiryasov2023BabyLlamaknowledgedistillation} was proved to be effective in BabyLM2023 and is included as one of the baselines officially provided by BabyLM2024. BabyLlama~\cite{timiryasov2023BabyLlamaknowledgedistillation}  employed knowledge distillation, transferring the knowledge from two teacher models — a GPT-2 model with 705 million parameters and a LLaMA model with 360 million parameters — into a compact BabyLlama “student” model with just 58 million parameters. Given that our own replication of the BabyLlama model through distillation did not achieve ideal results, we opted to use only the BabyLlama architecture  with a parameter size of 97 million. The BabyLlama model employs the classic CLM paradigm~\cite{gpt}, where given the first $n$ tokens in a sequence, the model predicts the token at position $n+1$. The next-token prediction (NTP) training objective is to minimize the negative log-likelihood loss of predicting the next token at each timestep. To achieve this, a causal mask is applied in the self-attention mechanism. This mask is represented as a lower triangular matrix, ensuring each token can only attend to its preceding tokens. Formally, for an input sequence of length $T$, $x_1, x_2, \dots, x_T$, the corresponding attention mask $M$ is a $T \times T$ lower triangular matrix, where $M_{ij} $ indicates whether the token at position $i$ should attend to the token at position $j$. 
This masking strategy effectively prevents the model from accessing future information during training, thereby capturing the sequential order and dependencies within the data.

\input{fig/fig_main}





% LTG-BERT结构+MLM目标 @guo
% 在2023年的babylm比赛中，Boot-Bert的实验和ELC-Bert的实验证明了LTG-BERT结构改进的有效性。LTG-BERT也是2024年babylm比赛官方提供的baselines之一。LTG-BERT的主要改进分别是NormFormer的层归一化，有相对位置的disentangled attention和门控线性激活函数GEGLU。LTG-BERT模型的训练目标主要是自监督训练目标——掩码语言建模（MLM）。通过随机选取其中的15%的token替换。这些被选择的token中，80%被遮蔽，10%被替换为随机的token，10%的不做处理。然后训练模型去预测原来的token。LTG-BERT研究了屏蔽文本单元的三种常见选择：Subwords，Whole words和Spans，发现基于跨度的遮蔽方法性能稍微好点。%
In  BabyLM2023~\cite{conll-2023-babylm}, experiments with Boot-BERT~\cite{samuel2023meanbootbert} and ELC-BERT~\cite{charpentier2023not} demonstrated the effectiveness of the LTG-BERT~\cite{samuel2023trained} architecture. LTG-BERT is also one of the official baselines in BabyLM2024. The LTG-BERT model incorporates several key architectural improvements, including NormFormer layer normalization~\cite{shleifer2021normformer}, disentangled attention with relative position embeddings~\cite{he2020deberta}, and gated-linear activation function~\cite{shazeer2020glu}. The training objective of LTG-BERT is self-supervised Masked Language Modeling (MLM). During training, 15\% of the tokens in the input sequence are randomly selected for replacement. Of these, 80\% are masked, 10\% are substituted with random tokens, and the remaining 10\% are unchanged. The model is then trained to predict the original masked tokens based on the context. LTG-BERT explores three common masking strategies: subwords, whole words, and spans. Experimental results indicate that span-based masking yields slightly better performance compared to the other methods.


\subsection{Our Approach}
\label{ssec:method}

% 基于两种基座，分别整合两个训练目标 @yu + @guo
%受到儿童通过完形填空练习和写作任务学习语言方式的启发，本研究基于两种不同的模型架构——BabyLlama 和 LTG-BERT，构建了一个统一的训练框架，整合了自回归语言模型 (CLM) 和掩码语言模型 (MLM) 两种训练目标。BabyLlama 作为自回归语言模型的代表，擅长序列生成任务。而 LTG-BERT 作为一种双向编码器模型，利用掩码机制捕捉双向的上下文依赖。在这一统一框架中，我们动态调整注意力掩码机制，使模型能够在 ALM 和 MLM 两种训练目标之间切换，并在评估阶段应用相应的掩码。自回归任务专注于下一个 token 的预测，使用因果掩码来确保序列依赖性。相比之下，掩码语言模型任务使用双向注意力，允许模型通过同时利用前后文来预测被掩盖的 token。通过结合这两种训练方式，模型不仅在序列生成任务（如文本生成）中表现出色，还通过双向注意力机制捕捉更广泛的上下文信息，从而在语言的语义理解上取得更深入的表现。%
Inspired by the way children learn languages through both cloze exercises and writing assignments, our work constructs a unified training framework that integrates CLM and MLM. In this unified framework, we switch between the two training paradigms alternately. CLM uses a causal mask to enforce sequential dependencies and MLM employs bidirectional attention, enabling the model to predict masked tokens by leveraging both preceding and succeeding context. By combining these two training objectives, the model not only excels at autoregressive tasks like text generation but also achieves a deeper semantic understanding of language by capturing broader contextual information through bidirectional attention. 

% move to exp
% while also applying the corresponding mask during the evaluation phase. 

% 实验中具体如何整合（交替）
% 我们集成MLM与CLM的方式是在预训练过程中切换训练目标。我们把模型在其中一个目标训练一定的轮次后，会切换到另一个目标。切换训练目标的方法是修改模型的输入和注意力矩阵。对于MLM任务，模型的输入会随机选择15%token进行替换。模型使用双向注意力根据上下文预测原有的token。对于CLM任务，模型的输入不需要进行token的替换。模型使用单向注意力根据前文预测下一个token。%
In our approach, we integrate CLM and MLM by alternating between these training objectives during the pre-training phase. After training the model on one objective for a specified number of epochs, we switch to the other objective. The switch between training objectives is implemented by modifying the model's input and attention matrix. For the MLM task, 15\% of the tokens in the input are randomly selected and replaced. The model utilizes bidirectional attention to predict the original tokens based on the surrounding context. In contrast, for the CLM task, no token replacement is required in the input. The model employs causal attention to predict the next token based on the preceding tokens.



==> arxiv/sec/5_experiment.tex <==

\section{Experiment}
\label{sec:exper}

\input{tab/hyperparameter}
\input{tab/main_results}

\paragraph{Data Preprocessing}
%关于数据的预处理部分，我们采用了去年在 Babylm Challenge 中表现突出的 BootBERT 方法中对数据的处理流程，其中包含对标点符号的规范化、重建句子结构和去除重复的文本等等。%
For the data preprocessing part, we adopt the data handling procedures from the BootBERT~\cite{samuel2023meanbootbert} method, which performed well in the previous round of BabyLM Challenge. Preprocessing includes steps like normalizing punctuation, reconstructing sentence structures, and removing duplicate text. These preprocessing steps help ensure cleaner and more structured input data, contributing to better model performance.

\paragraph{Baselines}
%我们直接采用了BabyLM挑战官方给出的Baseline作为我们自己的基准，即使用去年在这项任务中表现最优秀的模型LtgBERT与BabyLlama在测评数据集上取得的结果。具体的信息如表1所示%
We adopt the official baseline provided by the BabyLM Challenge as our benchmark, using the results achieved by the best-performing models from the previous round, namely LTG-BERT and BabyLlama, see Table~\ref{tab:main-result}.


\paragraph{Experiment Settings}
%在我们的实验中，我们分别使用 BabyLlama和LGT-BERT来研究结合自回归语言建模（CLM）和掩码语言建模（MLM）的混合训练策略的性能。两个模型基座，我们使用了相同的模型参数，具体模型的参数如表所示，且在训练中都使用AdamW 优化器进行优化，都使用 bfloat16 数据类型以提升计算效率。BabyLlama的批量大小为512，初始学习率设置为 7×10−4，在CLM训练模式阶段采用cosine调度器，在MLM训练模式阶段采用cosine with restarts调度器，scheduler num cycle设置为每四个epoch一个cycle。LGT-BERT的批量大小为1024，初始学习率设置为5×10−4，在所有的训练模式下面都采用cosine with restarts调度器，每个阶段的cycle设置为4。该模型经过多个周期的训练，交替进行 CLM 和 MLM 目标的训练。我们使用"x\textbackslash{}_CLM+y\textbackslash{}_MLM..."来表示按照先后顺序，在CLM训练模式下训练x个epoch，再在MLM训练模式下训练y个epoch，以此类推。 
In our experiments, we used both the BabyLlama and LGT-BERT models to evaluate the performance of a hybrid training strategy combining Causal Language Modeling (CLM) and Masked Language Modeling (MLM). For both model architectures, we used the same set of parameters, as shown in the table~\ref{tab:Hyper-parameter} and optimized the training process using the AdamW optimizer. Additionally, we employed the bfloat16 data type to enhance computational efficiency. For the BabyLlama model, we used a batch size of 512 with an initial learning rate set to $7 \times 10^{-4}$.  The learning rate scheduler followed a cosine decay during the CLM training phase and a cosine with restarts scheduler during the MLM phase, with the number of cycles set to every four epochs . For the LGT-BERT model, we employed a batch size of 1024, with an initial learning rate of $5 \times 10^{-4}$. In all training phases, we used a cosine with restarts scheduler, with the num cycles set to 4. Our hyperparameters were determined through multiple experiments, building upon the hyperparameter settings from the previous works~\cite{timiryasov2023BabyLlamaknowledgedistillation,samuel2023trained} to find the optimal values.
The training process alternated between CLM and MLM objectives over multiple epochs. We used the notation ``$x$\_CLM + $y$\_MLM..." to indicate that, \textit{in sequential order}, $x$ epochs are trained in the CLM training mode, followed by $y$ epochs in the MLM training mode, and so on.
 



\input{tab/main_experiment}
% \input{tab/main_ltg-bert}
\subsection{Main Results}
%在本节中，我们评估了 BabyLlama 和 LTG-BERT 在多个基准任务上的表现，包括 BLiMP、BLiMP Supplement、EWoK 和 GLUE。我们的实验主要聚焦于评估集成CLM和MLM训练目标对实验结果的影响，并对比了BabyLlama和LTG-BERT的基线与我们提出的配置。 
%通过表1我们可以看出，不管是在LTG-BERT模型上还是在BabyLlama模型上，我们集成了训练目标的模型整体上都超过了官方发布的baseline分数，而且在LTG-BERT上面取得了非常大的提升。
%为了进一步验证交替训练CLM和MLM两种目标的效果，我们在BabyLlama模型上进行了深入实验。鉴于在GLUE数据集上的训练时间较长，我们选择在BLiMP、BLiMP Supplement和EWoK数据集上进行评估。结果如表二显示，使用4\_CLM+16\_MLM+4\_CLM策略训练的模型整体性能显著优于单独使用8\_CLM或16\_MLM训练的模型。这一发现表明，将两种训练目标结合起来，可以使模型同时具备双向上下文理解和序列生成的能力。在相同的训练周期下，4\_CLM+16\_MLM+4\_CLM的组合再次表现出明显的优势，优于纯粹的24\_CLM或24\_MLM模型，进一步证明了这两种训练目标的结合是实现最佳性能的关键,，CLM和MLM之间形成了良好的互补关系。 
%此外，我们还探讨了这两种训练模式在不同数据集上的表现。如表2所示，MLM在EWoK数据集上的效果显著优于CLM，而CLM在BLiMP数据集上的表现则更加突出且敏感。这表明，不同的训练方式对不同数据集的影响存在差异，因此结合两种训练方式的集成实验能够更好地发挥其优势，提升整体效果。我们在图1中展示了一组完整的训练过程折线图来更加直观的表现上述现象。
\input{fig/fig_example}

In this section, we evaluate the performance of BabyLlama and LTG-BERT across multiple benchmarks, including BLiMP, BLiMP Supplement, EWoK, and GLUE. Our experiments primarily focus on assessing the impact of integrating CLM and MLM training objectives on the overall results, comparing the baseline performance of both BabyLlama and LTG-BERT with the configurations we propose. 

As shown in Table \ref{tab:main-result}, our models with integrated training objectives consistently outperform the official baseline scores on both the LTG-BERT and BabyLlama models. Notably, the improvements on LTG-BERT are particularly significant, demonstrating the effectiveness of our approach. 
To further validate the effectiveness of alternating training objectives CLM and MLM, we conducted an in-depth experiment with the BabyLlama model. Given the lengthy training times associated with the GLUE dataset, we opted to evaluate our results on the BLiMP, BLiMP Supplement, and EWoK datasets. As shown in Table \ref{tab:main-experiment}, the model trained with the \textit{4\_CLM+16\_MLM+4\_CLM} strategy significantly outperformed those trained solely with \textit{8\_CLM} or \textit{16\_MLM}. This finding indicates that combining these two training objectives enables the model to simultaneously acquire bidirectional context understanding and sequence generation capabilities. Under the same training epochs, the \textit{4\_CLM+16\_CLM+4\_CLM} combination demonstrated clear advantages over the pure \textit{24\_CLM} and \textit{24\_MLM} models, further confirming that the integration of these two training objectives is crucial for achieving optimal performance, highlighting the complementary relationship between CLM and MLM. We also conducted similar experiments on the LTG-BERT, the results are shown on same Table.


\input{tab/ablation}
 
Additionally, we explored the performance of these training modes across different datasets. As shown in Figure~\ref{fig:example}, MLM performs significantly better on the EWoK dataset, while CLM exhibits more pronounced and sensitive results on the BLiMP dataset. This indicates that different training approaches have varying impacts on distinct datasets. Thus, the integrated experiments that combine both training methods can better leverage their strengths and enhance overall performance. 


\subsection{Ablation Study}

% 为了探索集成实验各种因素对测评任务结果的影响，我们进行了对集成实验的交替次数和交替顺序两个变量的消融实验。具体来说，对于交替次数的实验，我们将同样epoch的训练过程从三阶段拆分成了更多阶段的训练，而对于交替顺序的实验，我们将三阶段实验中的MLM更改到了训练开始和结束的位置。%
% 实验结果如表4所示，这两个因素的变化不会导致测评结果有严重的下降，这也说明了我们的方法是稳定的。我们推测交替次数增多导致测评结果下降的原因可能是每个训练阶段epoch过小导致难以在对应训练任务上收敛。我们发现更改交替顺序导致的下降原因可能是CLM相比于MLM起到的作用更大，CLM是按顺序在每个token上都进行了预测训练，而MLM只是对mask掉的token进行了预测训练，因此我们推测CLM比MLM在一个epoch上面学到的东西要多，所以我们将CLM放在首尾
To investigate the effects of various factors on the evaluation task results within the integrated experiments, we conducted ablation studies focusing on two variables: alternating frequency and alternating order. In the BabyLlama model, we maintained a constant total number of training epochs at 24 (8 epochs for the CLM phase and 16 epochs for the MLM phase). Specifically, for the alternating order, we adjusted the alternating sequence of training between the CLM and MLM phases while keeping the overall epoch count unchanged. For alternating frequency, we divided the training process into more frequent alternating stages. 
The experimental results, as shown in Table \ref{tab:ab_bl}, indicate that variations in these two factors do not lead to significant declines in evaluation outcomes, suggesting that our approach is stable. We hypothesize that the decrease in performance with an increased frequency of alternations may be attributed to smaller epoch sizes in each training phase, which could hinder convergence on the respective tasks.

Furthermore, we found that the best performance was achieved when the CLM training phase was placed at both the beginning and the end of the training sequence, which could be due to the greater impact of CLM compared to MLM. Although CLM does not inherently have a higher performance ceiling (as last year’s winner was an MLM-based model), but it converges more rapidly. CLM performs sequential prediction training on every token, while MLM focuses only on masked tokens. Thus, we suggest that CLM captures more learning within a single epoch than MLM. 

 
% \subsection{Analysis}
% \subsection{Discussion}



==> arxiv/sec/6_conclusion.tex <==
\section{Conclusion}

% 最后写
% 在本研究中，我们提出了一个名为AntLM的模型，通过同时使用CLM和MLM两种任务交替训练来应对Babylm挑战中存在的多种自然语言相关的任务。实验结果表明，AntLM在所有任务测评中都取得了优于Baseline或与之相当的结果。
%我们发现CLMMLM两种训练任务对于不同的测评任务的影响不同，说明两种训练任务使得模型向不同的方向学习人类语言。我们认为这也是导致集成训练会有效果的主要原因，即模型能结合两种训练方式所学到的知识。这也引出了一个有趣的问题：不同的训练任务是否仅能使得模型学习到自然语言领域的一部分知识？由于资源的限制，我们未能在本研究中尝试更多的想法和方案。未来的研究中，我们计划在获得更多资源和支持后，进一步探索这些可能性。。
%除此之外，我们还进行了不同交替训练次数和顺序的相关实验，结果表明特定的集成训练方式在测评结果上是更有效的。
In this study, we propose AntLM, a model that applies to multiple natural language-related tasks in the BabyLM Challenge by alternating between Causal Language Modeling (CLM) and Masked Language Modeling (MLM) during training. Experimental results demonstrate that AntLM achieves either superior or comparable performance to the baseline across all evaluation tasks. 

Additionally, we found that CLM and MLM have different impacts on various evaluation tasks, suggesting that these training tasks guide the model to learn distinct aspects of human language. We believe this difference is the key reason why integrated training yields effective results, as the model benefits from the knowledge learned from both training approaches. This finding also raises an intriguing question: do different training tasks allow models to capture only specific portions of natural language knowledge? Due to resource limitations, we were unable to explore additional ideas and approaches in this study. In future work, we plan to address these limitations by expanding our resources and support, allowing us to further investigate these potential directions.

Moreover, we conducted experiments with varying numbers and sequences of alternating training, and the results suggest that specific integrated training methods are more effective in achieving optimal evaluation outcomes.

==> arxiv/tab/baselines.tex <==
\begin{table*}[ht]
    \centering
        \begin{tabular}{ccccccc}
        \toprule
        \textbf{Model}&\textbf{Data}&\textbf{BLiMP}&\textbf{BLiMP Supplement}&\textbf{EWoK}&\textbf{GLUE}&\textbf{\textit{Macroaverage}} \\
        \midrule
        LTG-BERT&10M&60.6&60.8&48.9&60.3&57.5 \\ 
        BabyLlama&100M&73.1&60.6&52.1&69.0&63.7 \\ 
        LTG-BERT&100M&69.2&66.5&51.9&68.4&64.0 \\
        \end{tabular}
    \caption{Baselines of LtgBERT and BabyLlama on evaluation datasets}
    \label{tab:baseline}
\end{table*}


==> arxiv/tab/hyperparameter.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{ccc}
		\toprule  % 顶部线
		\textbf{Name}&\textbf{BabyLlama}&\textbf{LTG-BERT} \\
		\midrule  % 中部线
		layers&12&12 \\
        attention heads&12&12\\ 
        hidden size&768&768\\
        intermediate size&2048&2048\\
        vocabulary size&16k&16k\\
        position bucket  & -- &32 \\
		\bottomrule  % 底部线
	\end{tabular}
\caption{Model Hyper-parameters.}
\label{tab:Hyper-parameter}
% \par \footnotesize
% Note: This is an example note written below the table using smaller font size.
\end{table}

==> arxiv/tab/main_results.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ccccccc}
        \toprule  % 顶部线
  \textbf{Model}&\textbf{Data}&\textbf{BLiMP}&\textbf{$\text{BLiMP}_\text{Supplement}$}&\textbf{EWoK}&\textbf{GLUE}&\textbf{\textit{Macro Avg.}} \\ 
        \midrule  % 中部线
        BabyLlama$^\dag$& 10M & \bf 69.8 & 59.5 & 50.7 & 63.3&60.8 \\
        BabyLlama& 10M &  68.1 & 60.4 & 50.4 & 65.5  &61.1 \\
        AntLM$_\text{BabyLlama}$ & 10M&69.4&\bf 60.7 &\bf 51.1 &\bf 67.4 & \bf 62.1 \\ 
        \midrule  % 中部线
        BabyLlama$^\dag$& 100M &  73.1 & 60.6 &\bf 52.1 & \bf69.0&63.7 \\
        LTG-BERT$^\dag$&100M&69.2&\bf 66.5&51.9&68.4&64.0 \\
         BabyLlama & 100M& \bf 74.9& 66.0 & 52.0 & 66.3 & \bf 64.8 \\
       
        \midrule
        LTG-BERT$^\dag$&10M&60.6&60.8&48.9&60.3&57.5 \\
        LTG-BERT&10M&62.6&\bf 65.4&62.3&64.9&63.8 \\
        AntLM$_\text{LTG-BERT}$ &10M&\bf 72.3&62.6 &  \bf 63.0 & \bf 66.0 & \bf 66.0 \\
        % \midrule
        % LTG-BERT$^\dag$&100M&69.2&66.5&51.9&68.4&64.0 \\
         % LTG-BERT$^\dag$ & 100M & 69.2 & 66.5&51.9 & 68.4 & 64.0 \\
         % AntLM$_\text{LTG-BERT}$ & 100M&  58.7& 62.0 & 65.3 &  65.2 & 62.8 \\
        \bottomrule  % 底部线
    \end{tabular}
    \caption{Main experimental results. The $^\dag$ indicates results from the official report. The official BabyLlama leverages knowledge distillation, while our AntLM$_\text{BabyLlama}$ is based solely on the architecture of BabyLlama without knowledge distillation methods. Due to limitations in time and resources, we have not attempted AntLM on the 100M track, this will be part of our future work. }
    \label{tab:main-result}
\end{table*}


==> tab/baselines.tex <==
\begin{table*}[ht]
    \centering
        \begin{tabular}{ccccccc}
        \toprule
        \textbf{Model}&\textbf{Data}&\textbf{BLiMP}&\textbf{BLiMP Supplement}&\textbf{EWoK}&\textbf{GLUE}&\textbf{\textit{Macroaverage}} \\
        \midrule
        LTG-BERT&10M&60.6&60.8&48.9&60.3&57.5 \\ 
        BabyLlama&100M&73.1&60.6&52.1&69.0&63.7 \\ 
        LTG-BERT&100M&69.2&66.5&51.9&68.4&64.0 \\
        \end{tabular}
    \caption{Baselines of LtgBERT and BabyLlama on evaluation datasets}
    \label{tab:baseline}
\end{table*}

